Improved model of the Supernova Refsdal cluster MACS J1149.5+2223 thanks to VLT/MUSE

We present new VLT/MUSE observations of the Hubble Frontier Field (HFF) galaxy cluster MACS J1149.5+2223, lensing the well-known supernova "Refsdal" into multiple images, which enabled the first cosmological applications with a strongly lensed supernova. Thanks to these data, targeting a northern region of the cluster and thus complementing our previous MUSE program on the cluster core, we release a new catalog containing 162 secure spectroscopic redshifts. We confirm 22 cluster members, which were previously only photometrically selected, and detect ten additional ones, resulting in a total of 308 secure members, of which 63% are spectroscopically confirmed. We further identify 17 new spectroscopic multiple images belonging to 6 different background sources. By exploiting MUSE data, in combination with the deep HFF images, we develop an improved total mass model of MACS J1149.5+2223. This model includes 308 total mass components for the member galaxies and requires four additional mass profiles, one of which is associated with a cluster galaxy overdensity identified in the North, representing the DM mass distribution on larger scales. The values of the resulting 34 free parameters are optimized based on the observed positions of 106 multiple images from 34 different families, that cover the redshift range between 1.240 and 5.983. Our final model has a multiple image position rms value of 0.39", which is well in agreement with that of other cluster lens models. With this refined mass model, we pave the way towards even better strong-lensing analyses that will exploit the deep and high resolution observations with HST and JWST on a pixel level in the region of the supernova Refsdal host. This will increase the number of observables by around two orders of magnitudes, thus offering us the opportunity of carrying out more precise and accurate cosmographic measurements.

==> table_clustermembers.tex <==

\begin{table}[ht!]
    \caption{List of cluster members.}
    \label{tab:clustermembers}
\end{table}
%
\tablefirsthead{%\multicolumn{4}{c}{Table 2: List of cluster members}\\ 
\toprule ID& R.A. & Decl. & F160W \\  & (J2000) & (J2000) & [mag] \\ \midrule }
%
\tablehead{%
\multicolumn{4}{c}%
{{\bfseries  Table~\ref{tab:clustermembers} Continued:} List of cluster members.} \\
\toprule
ID& R.A. & Decl. & F160W \\  & (J2000) & (J2000) & [mag] \\ \midrule}
%
%\tabletail{%
%\midrule \multicolumn{4}{r}{{Continued on next column}} \\ \midrule}
%\tablelasttail{%
%\\\midrule
%\multicolumn{4}{r}{{Concluded}} \\ \bottomrule}
\begin{xtabular}{cccc}
1 & 177.3731103 & 22.3929993 & $21.17 \pm 0.01$ \\ 
2 & 177.3749747 & 22.4045159 & $23.26 \pm 0.03$ \\ 
3 & 177.3761791 & 22.3916571 & $22.24 \pm 0.01$ \\ 
4 & 177.3764029 & 22.4004485 & $22.26 \pm 0.02$ \\ 
5 & 177.3765501 & 22.4052233 & $20.41 \pm 0.05$ \\ 
6 & 177.3766324 & 22.4020742 & $23.30 \pm 0.04$ \\ 
7 & 177.3769179 & 22.3946220 & $21.20 \pm 0.01$ \\ 
8 & 177.3776576 & 22.4031245 & $21.18 \pm 0.07$ \\ 
9 & 177.3777555 & 22.3940129 & $23.75 \pm 0.03$ \\ 
10 & 177.3787138 & 22.3928085 & $22.77 \pm 0.02$ \\ 
11 & 177.3793403 & 22.4089074 & $22.73 \pm 0.14$ \\ 
12 & 177.3794510 & 22.3838879 & $23.38 \pm 0.02$ \\ 
13 & 177.3796550 & 22.3995798 & $23.50 \pm 0.02$ \\ 
14 & 177.3797153 & 22.3950962 & $22.08 \pm 0.01$ \\ 
15 & 177.3798158 & 22.4070585 & $23.05 \pm 0.04$ \\ 
16 & 177.3798529 & 22.4084316 & $23.58 \pm 0.05$ \\ 
17 & 177.3801068 & 22.3833610 & $23.81 \pm 0.04$ \\ 
18 & 177.3805295 & 22.3978902 & $21.16 \pm 0.07$ \\ 
19 & 177.3810901 & 22.4011338 & $22.38 \pm 0.12$ \\ 
20 & 177.3816895 & 22.3969855 & $18.98 \pm 0.03$ \\ 
21 & 177.3822561 & 22.3968499 & $23.48 \pm 0.01$ \\ 
22 & 177.3824495 & 22.3986635 & $21.19 \pm 0.01$ \\ 
23 & 177.3825434 & 22.4071676 & $22.91 \pm 0.02$ \\ 
24 & 177.3827488 & 22.4130956 & $21.01 \pm 0.06$ \\ 
25 & 177.3827453 & 22.3902366 & $19.75 \pm 0.04$ \\ 
26 & 177.3829648 & 22.4069360 & $21.92 \pm 0.10$ \\ 
27 & 177.3831561 & 22.4159194 & $22.36 \pm 0.12$ \\ 
28 & 177.3833852 & 22.4005000 & $23.14 \pm 0.03$ \\ 
29 & 177.3835292 & 22.4149358 & $21.07 \pm 0.07$ \\ 
30 & 177.3835915 & 22.4107243 & $22.93 \pm 0.16$ \\ 
31 & 177.3837231 & 22.4170953 & $22.25 \pm 0.12$ \\ 
32 & 177.3839013 & 22.3997058 & $22.57 \pm 0.02$ \\ 
33 & 177.3839002 & 22.4102825 & $19.69 \pm 0.04$ \\ 
34 & 177.3839893 & 22.3847416 & $20.31 \pm 0.05$ \\ 
35 & 177.3840016 & 22.4066719 & $21.69 \pm 0.09$ \\ 
36 & 177.3840824 & 22.3941652 & $21.27 \pm 0.01$ \\ 
37 & 177.3841096 & 22.3938597 & $18.95 \pm 0.03$ \\ 
38 & 177.3843614 & 22.4093069 & $23.03 \pm 0.16$ \\ 
39 & 177.3846696 & 22.4149516 & $22.81 \pm 0.15$ \\ 
40 & 177.3846725 & 22.3870290 & $19.46 \pm 0.03$ \\ 
41 & 177.3846902 & 22.4028992 & $23.27 \pm 0.02$ \\ 
42 & 177.3847221 & 22.4004881 & $19.99 \pm 0.04$ \\ 
43 & 177.3847563 & 22.3998036 & $23.88 \pm 0.04$ \\ 
44 & 177.3848596 & 22.3988438 & $21.68 \pm 0.09$ \\ 
45 & 177.3851052 & 22.3967075 & $23.88 \pm 0.03$ \\ 
47 & 177.3863285 & 22.4035373 & $22.99 \pm 0.16$ \\ 
48 & 177.3863789 & 22.4137070 & $21.90 \pm 0.10$ \\ 
49 & 177.3866212 & 22.4136472 & $21.22 \pm 0.07$ \\ 
50 & 177.3867140 & 22.3771378 & $23.69 \pm 0.07$ \\ 
51 & 177.3870641 & 22.4110364 & $22.05 \pm 0.10$ \\ 
52 & 177.3873456 & 22.3989619 & $20.31 \pm 0.05$ \\ 
53 & 177.3874197 & 22.3946966 & $19.70 \pm 0.04$ \\ 
54 & 177.3875920 & 22.3875792 & $20.97 \pm 0.01$ \\ 
55 & 177.3875918 & 22.3870170 & $20.06 \pm 0.04$ \\ 
56 & 177.3876578 & 22.3808865 & $23.98 \pm 0.08$ \\ 
57 & 177.3877139 & 22.3937473 & $20.78 \pm 0.06$ \\ 
58 & 177.3878099 & 22.3953928 & $20.92 \pm 0.06$ \\ 
59 & 177.3880337 & 22.4118108 & $20.84 \pm 0.06$ \\ 
60 & 177.3881043 & 22.4137612 & $19.98 \pm 0.04$ \\ 
61 & 177.3881140 & 22.4084036 & $19.25 \pm 0.03$ \\ 
62 & 177.3882889 & 22.4022591 & $23.27 \pm 0.02$ \\ 
63 & 177.3883130 & 22.4116956 & $21.53 \pm 0.08$ \\ 
64 & 177.3884107 & 22.3932602 & $23.96 \pm 0.02$ \\ 
65 & 177.3884276 & 22.3999340 & $23.22 \pm 0.02$ \\ 
66 & 177.3887291 & 22.4003339 & $23.41 \pm 0.02$ \\ 
67 & 177.3888647 & 22.4141489 & $21.07 \pm 0.07$ \\ 
68 & 177.3889956 & 22.3847858 & $21.80 \pm 0.09$ \\ 
69 & 177.3891754 & 22.3820814 & $22.97 \pm 0.16$ \\ 
70 & 177.3894479 & 22.3926103 & $20.64 \pm 0.01$ \\ 
71 & 177.3894511 & 22.3939049 & $18.81 \pm 0.02$ \\ 
72 & 177.3894691 & 22.4063750 & $20.14 \pm 0.04$ \\ 
73 & 177.3896136 & 22.4167199 & $23.45 \pm 0.04$ \\ 
74 & 177.3896958 & 22.3927060 & $19.46 \pm 0.03$ \\ 
75 & 177.3901109 & 22.4157074 & $22.32 \pm 0.12$ \\ 
76 & 177.3901513 & 22.4038895 & $20.81 \pm 0.06$ \\ 
77 & 177.3902919 & 22.4139743 & $23.12 \pm 0.17$ \\ 
78 & 177.3903345 & 22.3807635 & $20.45 \pm 0.05$ \\ 
79 & 177.3905033 & 22.3853671 & $22.49 \pm 0.02$ \\ 
80 & 177.3907327 & 22.4094363 & $23.57 \pm 0.21$ \\ 
81 & 177.3909653 & 22.4016798 & $20.07 \pm 0.04$ \\ 
82 & 177.3910406 & 22.4032856 & $23.09 \pm 0.17$ \\ 
83 & 177.3910949 & 22.4049074 & $19.48 \pm 0.03$ \\ 
84 & 177.3912000 & 22.3927134 & $19.99 \pm 0.04$ \\ 
85 & 177.3913386 & 22.4077900 & $22.02 \pm 0.10$ \\ 
86 & 177.3913815 & 22.4010666 & $21.53 \pm 0.08$ \\ 
87 & 177.3914400 & 22.3795156 & $22.48 \pm 0.02$ \\ 
88 & 177.3916797 & 22.3906162 & $19.71 \pm 0.04$ \\ 
89 & 177.3918254 & 22.4052860 & $20.15 \pm 0.04$ \\ 
90 & 177.3921040 & 22.4034140 & $23.21 \pm 0.18$ \\ 
91 & 177.3921661 & 22.4012806 & $21.86 \pm 0.10$ \\ 
92 & 177.3921869 & 22.4147595 & $22.94 \pm 0.16$ \\ 
93 & 177.3925617 & 22.4105920 & $21.25 \pm 0.07$ \\ 
94 & 177.3926629 & 22.3927295 & $19.28 \pm 0.03$ \\ 
95 & 177.3926885 & 22.3943597 & $20.67 \pm 0.06$ \\ 
96 & 177.3927787 & 22.3980946 & $19.58 \pm 0.03$ \\ 
97 & 177.3928769 & 22.4181993 & $21.75 \pm 0.09$ \\ 
98 & 177.3928807 & 22.3970986 & $20.19 \pm 0.04$ \\ 
99 & 177.3929074 & 22.3930803 & $21.93 \pm 0.01$ \\ 
100 & 177.3929409 & 22.4118749 & $19.10 \pm 0.03$ \\ 
101 & 177.3931374 & 22.4113304 & $20.10 \pm 0.04$ \\ 
102 & 177.3933387 & 22.4104303 & $22.33 \pm 0.12$ \\ 
103 & 177.3934683 & 22.3798125 & $23.99 \pm 0.04$ \\ 
104 & 177.3934977 & 22.4204074 & $23.73 \pm 0.03$ \\ 
105 & 177.3936455 & 22.3948213 & $22.89 \pm 0.01$ \\ 
106 & 177.3938095 & 22.4023052 & $21.89 \pm 0.10$ \\ 
107 & 177.3938201 & 22.4116907 & $19.06 \pm 0.03$ \\ 
108 & 177.3940124 & 22.3953329 & $23.38 \pm 0.02$ \\ 
109 & 177.3940488 & 22.4084318 & $20.38 \pm 0.05$ \\ 
110 & 177.3940777 & 22.4127181 & $21.64 \pm 0.09$ \\ 
111 & 177.3941590 & 22.3950343 & $22.76 \pm 0.15$ \\ 
112 & 177.3942066 & 22.4124656 & $20.97 \pm 0.06$ \\ 
113 & 177.3942794 & 22.4075500 & $21.32 \pm 0.07$ \\ 
114 & 177.3942962 & 22.3842902 & $23.45 \pm 0.01$ \\ 
115 & 177.3945344 & 22.4006257 & $21.77 \pm 0.09$ \\ 
116 & 177.3946686 & 22.4133106 & $23.41 \pm 0.02$ \\ 
117 & 177.3946867 & 22.3786219 & $21.42 \pm 0.01$ \\ 
118 & 177.3947155 & 22.4113695 & $22.19 \pm 0.11$ \\ 
119 & 177.3947253 & 22.4144087 & $20.44 \pm 0.05$ \\ 
120 & 177.3948337 & 22.3929215 & $22.26 \pm 0.12$ \\ 
121 & 177.3950288 & 22.3960175 & $21.63 \pm 0.09$ \\ 
122 & 177.3950747 & 22.3898517 & $22.05 \pm 0.01$ \\ 
123 & 177.3951824 & 22.3818525 & $23.05 \pm 0.01$ \\ 
124 & 177.3952343 & 22.4149327 & $20.40 \pm 0.05$ \\ 
125 & 177.3952408 & 22.3969908 & $23.68 \pm 0.02$ \\ 
126 & 177.3952757 & 22.4010443 & $21.12 \pm 0.07$ \\ 
127 & 177.3954909 & 22.3876681 & $21.32 \pm 0.07$ \\ 
128 & 177.3957984 & 22.4182168 & $23.60 \pm 0.22$ \\ 
129 & 177.3958365 & 22.3934986 & $20.58 \pm 0.05$ \\ 
130 & 177.3960984 & 22.3840983 & $22.19 \pm 0.01$ \\ 
131 & 177.3965010 & 22.3979246 & $23.27 \pm 0.01$ \\ 
132 & 177.3965922 & 22.4133279 & $19.61 \pm 0.03$ \\ 
133 & 177.3967661 & 22.3837828 & $22.64 \pm 0.01$ \\ 
134 & 177.3967915 & 22.3784980 & $21.65 \pm 0.01$ \\ 
135 & 177.3968117 & 22.4100141 & $22.72 \pm 0.14$ \\ 
136 & 177.3968240 & 22.4107296 & $23.54 \pm 0.21$ \\ 
137 & 177.3968385 & 22.4174624 & $19.30 \pm 0.03$ \\ 
138 & 177.3968775 & 22.3923082 & $21.00 \pm 0.06$ \\ 
139 & 177.3969109 & 22.3777381 & $22.08 \pm 0.01$ \\ 
140 & 177.3969154 & 22.4180991 & $22.45 \pm 0.13$ \\ 
141 & 177.3969368 & 22.3929715 & $19.85 \pm 0.04$ \\ 
142 & 177.3970333 & 22.4115604 & $20.91 \pm 0.06$ \\ 
144 & 177.3972614 & 22.4002946 & $21.77 \pm 0.09$ \\ 
145 & 177.3973707 & 22.3896101 & $21.74 \pm 0.01$ \\ 
146 & 177.3975213 & 22.3995266 & $19.67 \pm 0.04$ \\ 
147 & 177.3976178 & 22.4028769 & $22.02 \pm 0.10$ \\ 
148 & 177.3976806 & 22.4161858 & $21.47 \pm 0.08$ \\ 
149 & 177.3977147 & 22.4152145 & $21.22 \pm 0.07$ \\ 
150 & 177.3977837 & 22.3954646 & $19.67 \pm 0.04$ \\ 
151 & 177.3979093 & 22.3970894 & $23.44 \pm 0.01$ \\ 
152 & 177.3979200 & 22.4039366 & $22.24 \pm 0.11$ \\ 
153 & 177.3979562 & 22.4010445 & $19.32 \pm 0.03$ \\ 
154 & 177.3979793 & 22.4045753 & $23.04 \pm 0.16$ \\ 
155 & 177.3981366 & 22.4159565 & $22.23 \pm 0.11$ \\ 
156 & 177.3981566 & 22.4074085 & $19.72 \pm 0.04$ \\ 
157 & 177.3981975 & 22.4162785 & $21.32 \pm 0.07$ \\ 
158 & 177.3982642 & 22.4107878 & $19.29 \pm 0.03$ \\ 
159 & 177.3983023 & 22.4031361 & $23.16 \pm 0.02$ \\ 
160 & 177.3983064 & 22.4160166 & $22.57 \pm 0.13$ \\ 
161 & 177.3984562 & 22.4053606 & $21.59 \pm 0.08$ \\ 
162 & 177.3985470 & 22.3897485 & $21.17 \pm 0.07$ \\ 
163 & 177.3986018 & 22.3980800 & $20.93 \pm 0.06$ \\ 
164 & 177.3986059 & 22.4071693 & $23.01 \pm 0.02$ \\ 
165 & 177.3987043 & 22.3923060 & $20.18 \pm 0.04$ \\ 
166 & 177.3987444 & 22.3985302 & $17.95 \pm 0.02$ \\ 
167 & 177.3988614 & 22.4018114 & $20.69 \pm 0.06$ \\ 
168 & 177.3990006 & 22.4183923 & $20.23 \pm 0.05$ \\ 
169 & 177.3990113 & 22.3801933 & $20.08 \pm 0.04$ \\ 
170 & 177.3991900 & 22.4009000 & $22.95 \pm 0.16$ \\ 
171 & 177.3992874 & 22.3814209 & $19.15 \pm 0.01$ \\ 
172 & 177.3993498 & 22.4132984 & $22.74 \pm 0.14$ \\ 
173 & 177.3994298 & 22.4154432 & $19.41 \pm 0.03$ \\ 
174 & 177.3994979 & 22.4122791 & $22.56 \pm 0.13$ \\ 
175 & 177.3995956 & 22.4023101 & $23.20 \pm 0.02$ \\ 
176 & 177.3996188 & 22.4209107 & $22.87 \pm 0.15$ \\ 
177 & 177.3996525 & 22.3996069 & $21.03 \pm 0.07$ \\ 
178 & 177.3997643 & 22.4184698 & $22.56 \pm 0.02$ \\ 
179 & 177.3998043 & 22.4149037 & $19.19 \pm 0.03$ \\ 
180 & 177.3998272 & 22.3972567 & $19.45 \pm 0.03$ \\ 
181 & 177.4001882 & 22.3792347 & $23.96 \pm 0.05$ \\ 
182 & 177.4001513 & 22.3944396 & $22.74 \pm 0.14$ \\ 
183 & 177.4002180 & 22.3979357 & $21.30 \pm 0.01$ \\ 
184 & 177.4004049 & 22.3982050 & $21.59 \pm 0.08$ \\ 
185 & 177.4007815 & 22.3962462 & $21.69 \pm 0.09$ \\ 
186 & 177.4007996 & 22.3937721 & $22.73 \pm 0.14$ \\ 
187 & 177.4010292 & 22.3978791 & $19.44 \pm 0.03$ \\ 
188 & 177.4011996 & 22.4003301 & $19.70 \pm 0.04$ \\ 
189 & 177.4012619 & 22.4156000 & $23.10 \pm 0.02$ \\ 
190 & 177.4012685 & 22.4188672 & $20.71 \pm 0.06$ \\ 
191 & 177.4013880 & 22.4109958 & $23.48 \pm 0.03$ \\ 
192 & 177.4015946 & 22.4113035 & $21.45 \pm 0.08$ \\ 
193 & 177.4016493 & 22.4094727 & $22.40 \pm 0.12$ \\ 
194 & 177.4017202 & 22.3987997 & $21.79 \pm 0.09$ \\ 
195 & 177.4020951 & 22.3778965 & $23.34 \pm 0.03$ \\ 
196 & 177.4021613 & 22.3828349 & $23.68 \pm 0.22$ \\ 
197 & 177.4022603 & 22.3997466 & $20.29 \pm 0.05$ \\ 
198 & 177.4022732 & 22.4112574 & $23.03 \pm 0.03$ \\ 
199 & 177.4023827 & 22.3980282 & $22.65 \pm 0.14$ \\ 
200 & 177.4024180 & 22.3760338 & $22.79 \pm 0.02$ \\ 
201 & 177.4025297 & 22.4104588 & $20.96 \pm 0.06$ \\ 
202 & 177.4025336 & 22.4188811 & $21.43 \pm 0.08$ \\ 
203 & 177.4026353 & 22.3962208 & $20.22 \pm 0.05$ \\ 
204 & 177.4026778 & 22.3964367 & $22.89 \pm 0.01$ \\ 
205 & 177.4026846 & 22.3787119 & $23.08 \pm 0.03$ \\ 
206 & 177.4028907 & 22.4020176 & $22.04 \pm 0.10$ \\ 
207 & 177.4029141 & 22.3779117 & $21.60 \pm 0.01$ \\ 
208 & 177.4029303 & 22.4116767 & $21.72 \pm 0.09$ \\ 
209 & 177.4030652 & 22.4043833 & $20.51 \pm 0.05$ \\ 
210 & 177.4031519 & 22.4144805 & $22.71 \pm 0.01$ \\ 
211 & 177.4033153 & 22.3972003 & $23.86 \pm 0.02$ \\ 
212 & 177.4034364 & 22.3778866 & $21.52 \pm 0.01$ \\ 
213 & 177.4035753 & 22.3963821 & $18.88 \pm 0.02$ \\ 
214 & 177.4035854 & 22.4055993 & $23.03 \pm 0.16$ \\ 
215 & 177.4036642 & 22.3919421 & $20.27 \pm 0.05$ \\ 
216 & 177.4036702 & 22.3940640 & $23.79 \pm 0.03$ \\ 
217 & 177.4036785 & 22.3883950 & $21.21 \pm 0.07$ \\ 
218 & 177.4036951 & 22.3891072 & $19.99 \pm 0.04$ \\ 
219 & 177.4037163 & 22.4045720 & $19.64 \pm 0.03$ \\ 
220 & 177.4038490 & 22.3890961 & $23.06 \pm 0.01$ \\ 
221 & 177.4040050 & 22.4021332 & $22.22 \pm 0.11$ \\ 
222 & 177.4040314 & 22.4030213 & $21.50 \pm 0.08$ \\ 
223 & 177.4040496 & 22.3863782 & $19.93 \pm 0.04$ \\ 
224 & 177.4041238 & 22.3853297 & $21.63 \pm 0.09$ \\ 
225 & 177.4045854 & 22.3964327 & $23.06 \pm 0.02$ \\ 
226 & 177.4047291 & 22.3822249 & $20.63 \pm 0.05$ \\ 
227 & 177.4048435 & 22.4167925 & $22.29 \pm 0.02$ \\ 
228 & 177.4049607 & 22.4108680 & $23.31 \pm 0.02$ \\ 
229 & 177.4051302 & 22.3980756 & $23.99 \pm 0.02$ \\ 
230 & 177.4051659 & 22.3997696 & $21.83 \pm 0.09$ \\ 
231 & 177.4053588 & 22.3916404 & $22.37 \pm 0.12$ \\ 
232 & 177.4054365 & 22.3978677 & $19.62 \pm 0.03$ \\ 
233 & 177.4060086 & 22.4088909 & $23.03 \pm 0.02$ \\ 
234 & 177.4060199 & 22.3810427 & $22.02 \pm 0.01$ \\ 
235 & 177.4061199 & 22.3991159 & $22.86 \pm 0.01$ \\ 
236 & 177.4062887 & 22.4054011 & $21.69 \pm 0.09$ \\ 
237 & 177.4063248 & 22.4065687 & $22.10 \pm 0.02$ \\ 
238 & 177.4064553 & 22.3895796 & $18.08 \pm 0.02$ \\ 
239 & 177.4066159 & 22.4044961 & $23.87 \pm 0.02$ \\ 
240 & 177.4066393 & 22.3955515 & $21.37 \pm 0.08$ \\ 
241 & 177.4067443 & 22.3874517 & $20.59 \pm 0.05$ \\ 
242 & 177.4068979 & 22.3958173 & $20.63 \pm 0.05$ \\ 
243 & 177.4071516 & 22.3866876 & $23.35 \pm 0.03$ \\ 
244 & 177.4072580 & 22.3914431 & $22.41 \pm 0.12$ \\ 
245 & 177.4072689 & 22.3978938 & $23.46 \pm 0.02$ \\ 
246 & 177.4073728 & 22.3947979 & $23.72 \pm 0.23$ \\ 
247 & 177.4074731 & 22.3991192 & $22.57 \pm 0.13$ \\ 
248 & 177.4075168 & 22.4030505 & $18.72 \pm 0.02$ \\ 
249 & 177.4083421 & 22.4077179 & $20.34 \pm 0.05$ \\ 
250 & 177.4084952 & 22.3932109 & $21.47 \pm 0.08$ \\ 
251 & 177.4088721 & 22.3966419 & $23.82 \pm 0.02$ \\ 
252 & 177.4090917 & 22.4155019 & $20.83 \pm 0.06$ \\ 
253 & 177.4092139 & 22.3943753 & $22.75 \pm 0.02$ \\ 
254 & 177.4094536 & 22.3953620 & $22.23 \pm 0.01$ \\ 
255 & 177.4095110 & 22.3928438 & $20.99 \pm 0.06$ \\ 
256 & 177.4098839 & 22.3978357 & $22.45 \pm 0.01$ \\ 
257 & 177.4099897 & 22.4135067 & $20.19 \pm 0.04$ \\ 
258 & 177.4101231 & 22.3894002 & $19.83 \pm 0.04$ \\ 
259 & 177.4101254 & 22.4001909 & $23.58 \pm 0.03$ \\ 
260 & 177.4104440 & 22.3840363 & $19.71 \pm 0.04$ \\ 
261 & 177.4104236 & 22.3859291 & $23.12 \pm 0.17$ \\ 
262 & 177.4104718 & 22.3802392 & $21.59 \pm 0.01$ \\ 
263 & 177.4105236 & 22.4078497 & $23.48 \pm 0.02$ \\ 
264 & 177.4106388 & 22.3951257 & $21.40 \pm 0.01$ \\ 
265 & 177.4107054 & 22.3858962 & $19.49 \pm 0.03$ \\ 
266 & 177.4117862 & 22.3904996 & $22.28 \pm 0.01$ \\ 
267 & 177.4118175 & 22.3960473 & $21.59 \pm 0.08$ \\ 
268 & 177.4118688 & 22.3824242 & $19.37 \pm 0.03$ \\ 
269 & 177.4120084 & 22.3976056 & $21.15 \pm 0.01$ \\ 
270 & 177.4122024 & 22.3833070 & $18.52 \pm 0.02$ \\ 
271 & 177.4125167 & 22.3825137 & $22.48 \pm 0.02$ \\ 
272 & 177.4128799 & 22.3912155 & $21.77 \pm 0.01$ \\ 
273 & 177.4128865 & 22.3936520 & $21.25 \pm 0.07$ \\ 
274 & 177.4131885 & 22.4161900 & $23.81 \pm 0.03$ \\ 
275 & 177.4132816 & 22.3999571 & $22.90 \pm 0.02$ \\ 
276 & 177.4134493 & 22.4127773 & $23.65 \pm 0.03$ \\ 
277 & 177.4137937 & 22.3979139 & $21.01 \pm 0.06$ \\ 
278 & 177.4138353 & 22.4084526 & $18.76 \pm 0.02$ \\ 
279 & 177.4140679 & 22.3836159 & $20.16 \pm 0.04$ \\ 
280 & 177.4142436 & 22.4140176 & $23.06 \pm 0.03$ \\ 
281 & 177.4142944 & 22.3902735 & $22.42 \pm 0.02$ \\ 
282 & 177.4146401 & 22.3943228 & $19.99 \pm 0.04$ \\ 
283 & 177.4148551 & 22.3848183 & $22.98 \pm 0.02$ \\ 
284 & 177.4152354 & 22.4023055 & $23.64 \pm 0.03$ \\ 
285 & 177.4159316 & 22.3969462 & $22.90 \pm 0.01$ \\ 
286 & 177.4162482 & 22.3923325 & $20.34 \pm 0.05$ \\ 
287 & 177.4162836 & 22.3895150 & $22.47 \pm 0.04$ \\ 
288 & 177.4173468 & 22.4011222 & $19.19 \pm 0.03$ \\ 
289 & 177.4174855 & 22.3998000 & $18.94 \pm 0.03$ \\ 
290 & 177.4175736 & 22.3907093 & $23.60 \pm 0.06$ \\ 
291 & 177.4178041 & 22.4151810 & $19.94 \pm 0.01$ \\ 
292 & 177.4181675 & 22.4073768 & $22.36 \pm 0.01$ \\ 
293 & 177.4181914 & 22.3993326 & $20.34 \pm 0.01$ \\ 
294 & 177.4186364 & 22.3895934 & $19.15 \pm 0.03$ \\ 
295 & 177.4186895 & 22.4157271 & $21.49 \pm 0.01$ \\ 
296 & 177.4190526 & 22.4053722 & $23.78 \pm 0.03$ \\ 
297 & 177.4199083 & 22.4067096 & $22.96 \pm 0.02$ \\ 
298 & 177.4201364 & 22.3944230 & $21.71 \pm 0.09$ \\ 
299 & 177.4207777 & 22.3900937 & $19.21 \pm 0.01$ \\ 
300 & 177.4223658 & 22.4032877 & $23.42 \pm 0.02$ \\ 
301 & 177.3975732 & 22.4093797 & $23.41 \pm 0.20$ \\ 
302 & 177.3899345 & 22.4096336 & $22.74 \pm 0.14$ \\ 
303 & 177.3804467 & 22.3811633 & $18.74 \pm 0.02$ \\ 
304 & 177.3769120 & 22.4116309 & $20.16 \pm 0.04$ \\ 
305 & 177.4179422 & 22.3855183 & $20.58 \pm 0.05$ \\ 
306 & 177.3990736 & 22.4224584 & $19.38 \pm 0.03$ \\ 
307 & 177.3992580 & 22.4059414 & $22.61 \pm 0.14$ \\ 
308 & 177.3881528 & 22.4193269 & $21.63 \pm 0.09$ \\ 
309 & 177.4006908 & 22.4086049 & $23.23 \pm 0.18$ \\ 
310 & 177.3825754 & 22.4165198 & $22.89 \pm 0.16$ \\ 
\end{xtabular}


%\noalign{\smallskip} \hline \\
%\noalign{\textbf{Note.} Columns give from left to right the identification number ID (following \citetalias{grillo16}), right ascension, declination, magnitude with uncertainty of the \textit{HST} F160W filter.}




==> table_further_sources.tex <==
\onecolumn
\begin{longtable}{cccccccc}
\caption{Possible additional multiply lensed images (adapted Tab.~3 of \citet{treu16}).}\\
\hline \hline \noalign{\smallskip}
ID & R.A.  & Decl. & $z$ & $\sigma_z$ & Score & Category & Grade \\
& (J2000) & (J2000) & & & & & \\
  \endfirsthead
  \caption*{\textbf{Table \ref{tab:additional_images} Continued:} Possible additional multiply lensed images.}\\
ID & R.A.  & Decl. & $z$ & $\sigma_z$ & Score & Category & Grade \\
& (J2000) & (J2000) & & & & & \\
  \hline
  \endhead
\noalign{\smallskip} \hline \noalign{\smallskip}
%1.1 & 177.39700 & 22.396000 & 1.488 & 1.0 & Gold \\
%1.2 & 177.39942 & 22.397439 & 1.488 & 1.0 & Gold \\
%1.3 & 177.40342 & 22.402439 & 1.488 & 1.0 & Gold \\
%1.5 & 177.39986 & 22.397133 &\nodata& 2.0 &\nodata \\
%2.1 & 177.40242 & 22.389750 & 1.891 & 1.0 & Gold \\
%2.2 & 177.40604 & 22.392478 & 1.891 & 1.0 & Gold \\
%2.3 & 177.40658 & 22.392886 & 1.891 & 1.0 & Gold \\
%3.1 & 177.39075 & 22.399847 & 3.129 & 1.0 & Gold \\
%3.2 & 177.39271 & 22.403081 & 3.129 & 1.0 & Gold \\
%3.3 & 177.40129 & 22.407189 & 3.129 & 1.1 & Gold \\
%4.1 & 177.39300 & 22.396825 & 2.949 & 1.0 & Gold \\
%4.2 & 177.39438 & 22.400736 & 2.949 & 1.0 & Gold \\
%4.3 & 177.40417 & 22.406128 & 2.949 & 1.0 & Gold \\
%5.1 & 177.39975 & 22.393061 & 2.800 & 1.0 & Gold \\
%5.2 & 177.40108 & 22.393825 &\nodata& 1.0 & Gold \\
5.3 & 177.40792 & 22.403553 & 2.787 & 0.03 & 1.7 & Silver & 2\\
%6.1 & 177.39971 & 22.392544 &\nodata& 1.1 & Gold \\
%6.2 & 177.40183 & 22.393858 &\nodata& 1.1 & Gold \\
6.3 & 177.40804 & 22.402506 & 3.0035 & 0.10 & 1.7 & Silver & 1\\
%7.1 & 177.39896 & 22.391339 &\nodata& 1.1 & Gold \\
%7.2 & 177.40342 & 22.394269 &\nodata& 1.1 & Gold \\
%7.3 & 177.40758 & 22.401242 &\nodata& 1.2 & Gold \\
%8.1 & 177.39850 & 22.394350 &\nodata& 1.2 & Gold \\
%8.2 & 177.39979 & 22.395044 &\nodata& 1.2 & Gold \\
%8.4 & 177.40709 & 22.404722 &\nodata& 1.2 & Gold \\
%\nodata& 177.40704 & 22.405553 & 2.780 & 3.0 & Rejected \\
%\nodata& 177.40517 & 22.401563 &\nodata& 3.0 & Rejected \\
9.1 & 177.40517 & 22.426233 &\nodata&\nodata& 1.8 &\nodata & 2\\ %29|35
9.2 & 177.40388 & 22.427231 &\nodata&\nodata& 1.8 &\nodata & 2\\
9.3 & 177.40325 & 22.427228 &\nodata&\nodata& 1.8 &\nodata & 2\\
9.4 & 177.40364 & 22.426422 &\nodata&\nodata& 1.8 &\nodata & 2\\
10.1& 177.40450 & 22.425514 &1.2678 & 0.576 & 1.8 &\nodata & 2\\ %30|36
10.2& 177.40362 & 22.425636 &\nodata&\nodata& 1.8 &\nodata & 2\\
10.3& 177.40221 & 22.426625 &\nodata&\nodata& 1.8 &\nodata & 2\\
%12.1& 177.39857 & 22.389356 & 1.020 & 2.6 & Rejected \\
%12.2& 177.40375 & 22.392345 & 0.929 & 2.9 & Rejected \\
%12.3& 177.40822 & 22.398801 & 1.118 & 2.6 & Rejected \\
%13.1& 177.40371 & 22.397786 & 1.230 & 1.0 & Gold \\
%13.2& 177.40283 & 22.396656 & 1.250 & 1.0 & Gold \\
%13.3& 177.40004 & 22.393858 & 1.230 & 1.3 & Gold \\
%14.1& 177.39167 & 22.403489 & 3.703 & 1.3 & Gold \\
%14.2& 177.39083 & 22.402647 & 3.703 & 1.3 & Gold \\
%110.1&177.40014 & 22.390162 & 3.214 & 1.0 & Gold \\
%110.2&177.40402 & 22.392894 & 3.214 & 1.0 & Gold \\
110.3&177.40907 & 22.400242 & 2.9 & 0.016 & 2.0 &\nodata & 1\\
21.1 &177.40451 & 22.386704 &\nodata&\nodata& 1.8 & Silver & 2\\ %31|37
21.2 &177.40800 & 22.389057 & 2.515 / 2.44 & 0.76 / 0.69 & 1.6 & Silver & 2\\
21.3 &177.40907 & 22.390407 & 1.882 & 0.93 & 1.6 & Silver & 2\\
22.1 &177.40370 & 22.386838 & 0.7734 & 0.02 & 1.8 &\nodata & 0\\ %32|38
22.2 &177.40791 & 22.389232 & 0.4873 & 0.01 & 1.8 &\nodata & 0\\
22.3 &177.40902 & 22.391053 & 0.588  & 0.04 & 1.8 &\nodata & 0\\
23.1 &177.39302 & 22.411428 &\nodata&\nodata& 1.8 &\nodata & 2\\ %33|39
23.2 &177.39308 & 22.411455 & 2.374 & 0.72 & 1.8 &\nodata & 2\\
23.3 &177.39315 & 22.411473 &\nodata&\nodata& 1.8 &\nodata & 2\\
%24.1 &177.39285 & 22.412872 &\nodata& 1.7 &\nodata \\
%24.2 &177.39353 & 22.413071 &\nodata& 1.7 &\nodata \\
%24.3 &177.39504 & 22.412697 &\nodata& 1.8 &\nodata \\
25.1 &177.40428 & 22.398782 & 1.151 & 0.001 & 2.0 &\nodata & 0 \\ %34|40
25.2 &177.40411 & 22.398599 & 0.7715 & 0.085 & 2.0 &\nodata& 0 \\
25.3 &177.39489 & 22.391796 & 4.105 & 0.02 & 2.3 &\nodata  & 0 \\
26.1 &177.41035 & 22.388749 & 3.1495 & 0.05 & 1.8 & Silver & 2\\ %35|41
26.2 &177.40922 & 22.387697 & 3.058 & 0.05 & 1.8 & Silver & 2\\
26.3 &177.40623 & 22.385369 & 3.19 & 0.075 & 1.8 & Silver & 2\\
27.1 &177.40971 & 22.387665 & 2.765 & 0.04 & 1.8 & Silver &2\\ %36|42
27.2 &177.40988 & 22.387835 & 2.76 & 0.04 & 1.8 & Silver &2\\
27.3 &177.40615 & 22.385142 & 1.1615 / 0.04 & 0.5 / 0.19 & 2.5 &\nodata &0\\
%28.1 &177.39531 & 22.391809 &\nodata& 2.0 &\nodata \\
%28.2 &177.40215 & 22.396750 &\nodata& 2.2 &\nodata \\
%28.3 &177.40562 & 22.402434 &\nodata& 2.0 &\nodata \\
200.1&177.40875 & 22.394467 & 2.3189 & 0 & 2.6 &\nodata &0\\ %37|43
200.2&177.40512 & 22.391261 & 2.987 & 0 & 2.6 &\nodata &0\\
200.3&177.40256 & 22.389233 &\nodata&\nodata& 2.8 &\nodata &1\\
201.1&177.40048 & 22.395444 & 2.8 & 0.864 & 1.6 &\nodata & 2\\ %38|44
201.2&177.40683 & 22.404517 & 2.772 & 0.02 & 1.6 &\nodata & 2\\
202.1&177.40765 & 22.396789 & 2.5415 & 0.047 & 2.0 &\nodata &2\\ %39|45
202.2&177.40224 & 22.391489 & 2.2496 & 0.077 & 2.0 &\nodata & 2 \\
202.3&177.40353 & 22.392586 &\nodata&\nodata& 2.0 &\nodata & 2\\
203.1&177.40995 & 22.387244 & 4.34 & 0.035 & 1.8 & Silver & 2\\ %40|46
203.2&177.40657 & 22.384511 & 5.01 & 0.02 & 2.0 & Silver & 2\\
203.3&177.41123 & 22.388461 & 4.775 & 2 & 1.8 & Silver & 2\\
204.1&177.40961 & 22.386661 & 0.415 & 0.06 & 1.8 & Silver & 1\\%41|47
204.2&177.40668 & 22.384322 & 6.556 & 0.133 & 1.8 & Silver & 2\\
204.3&177.41208 & 22.389056 & 6.68 & 0.094 & 1.8 & Silver & 2\\
205.1&177.40520 & 22.386042 & 1.76 & 1.384 & 2.0 &\nodata &1\\ %42|48
205.2&177.40821 & 22.388119 & 3.054 & 0 & 2.0 &\nodata &1\\
205.3&177.41038 & 22.390625 & 3.0185 & 0.076 & 2.0 &\nodata &1\\
206.1&177.40764 & 22.385647 & 0.7082 & 0.26 & 2.2 &\nodata &0 \\
206.2&177.40863 & 22.386453 & 3.005 & 0.781 & 2.2 &\nodata &1 \\ %43|49
206.3&177.41133 & 22.388997 & 3.017 & 0.095 & 2.2 &\nodata &1 \\
207.1&177.40442 & 22.397303 & 1.1601 & 0.1 & 2.2 &\nodata &2 \\ %44|50
207.2&177.40397 & 22.396039 & 1.699 & 0.37 & 2.2 &\nodata &2 \\
208.1&177.40453 & 22.395761 & 1.369 & 0 & 2.0 &\nodata & 3\\ %45|51
208.2&177.40494 & 22.396397 &\nodata&\nodata& 2.0 &\nodata & 3\\
209.1&177.38994 & 22.412694 & 9.559 & 3.635 & 3.0 &\nodata & 0\\ %46|52
209.2&177.39055 & 22.413408 & 8.62 & 3.189 & 3.0 &\nodata & 0 \\
210.1&177.39690 & 22.398061 & 0.702 & 0 & 3.0 &\nodata & 2 \\ %47|53
210.2&177.39505 & 22.397497 & 0.8 (0.702) & 0.029 (0) & 3.0 &\nodata & 2\\
501.1&177.40720 & 22.386880 &\nodata&\nodata&\nodata&\nodata&1\\ %48|54
501.2&177.40719 & 22.386967 &\nodata&\nodata&\nodata&\nodata&1\\
501.3&177.40712 & 22.387038 &\nodata&\nodata&\nodata&\nodata&1\\
501.4&177.40700 & 22.386880 &\nodata&\nodata&\nodata&\nodata&1\\
%\noalign{\smallskip} \hline \\
\label{tab:additional_images}
\end{longtable}
Note: Score and Category from Tab.~3 of \citet{treu16}. Grade means: 0=for sure not lensed, 1=possible but unlikely, 2=possible and likely, 3=likely to be a lensing system; according to redshifts, the model from \citetalias{grillo16}, and preliminary model.
\twocolumn

Notes:
\begin{itemize}
    \item[5.3:] not predicted by the G16 model but redshift very similar (2.8 for 5.1 and 5.2)
    \item[6.3:] not predicted by the G16 model
    \item[9:] not a system based on G16 model but also no mass so far out, only one redshift available so no constrain here.
    \item[10:] not a system based on G16 model and new model (z=1.489) but also no mass so far at this region, only one redshift available so no constrain here.
    \item[110.3:] 110.3 not predicted by the G16 model, redshift is 3.216 for 110.1 ans 110.2 and thus not matching those from 110.3 (but not too far away for photo-z)
    \item[21:] not matching in G16 model, redshifts (if available) differ but within 1 sigma. Relative good matching in new model (z=4), but not so good anymore at z=3.
    \item[22:] unlikely based on G16 model and new (at z=1.489), redshifts not matching, relative high Score.
    \item[23:] probable match based on G16 model, only one redshift available i.e. no possiblility to compare/judge based on the redshift. Score also relative good with 1.8 (although not in Silver)
    \item[25:] based on G16 modle no, redshifts are very different
    \item[26:] based on G16 model unlikely, counterimages quite a bit off in new model (z=3), redshifts similar
    \item[27:] based on G16 model 27.1 and 27.2 on the same arc and 27.1 and 27.2 have same redshifts. Based on new model (z=1.489) 207.1 and 207.2 not multiple images. 207.3 not a corresponding image.
    \item[200:] 200.1 and 200.2 have different spec-z.
    \item[201:] unclear from G16 model, redshifts match well.
    \item[202:] based on G16 model maybe yes, redshifts not completely matching but similar, as long as available.
    \item[203:] redshifts not matching but similar and such high photo-z not so trustworthy. Long stretched arc based on G16 model, not completely covering the knots. Long stretched arc on 203.1 with new model (z=5), nearly up to 203.3 but not including 203.2. Based on new model (z=4) still stretched arc but clearly no counter images. Member of the Silver sample.
    \item[204:] 204.1 based on G16 and new (z=6) model long arc nearly including 204.3 (but not vice versa), but redshift far away from those of 204.2 and 204.3; 204.2 and 204.3: based on G16 model not but based on redhsift possible. Not a image system based on new model (z=1.489 or z=6)
    \item[205:] no based on G16 model, possible based on redshifts
    \item[206:] 206.1 not based on G16 model, redshifts differ significantly. 206.2: and 206.3 very similar redshift but no based on G16 model. No image system based on new model (z=1.489).
    \item[207:] possible based on G16 model and new model (z=1.489), redshifts differ significantly
    \item[208:] based on G16 model yes and possible from new model (z=1.489), only one redshift available
    \item[209:] not based on G16 and new (z=9) model but models not good in this region, possible from the redshift. 209.1 correspond to the object from \citet{hashimoto18} at redshift 9.1096.
    \item[210:] no based on \citetalias{grillo16} model and new model (z=1.489), redhsift is the same in \citet{treu16} and similar in astrodeep catalog.
    \item[501:] hard to say from model, would need to include specific lens mass.
\end{itemize}
